AirSync: Enabling Distributed Multiuser MIMO with Full Spatial Multiplexing

The enormous success of advanced wireless devices is pushing the demand for higher wireless data rates. Denser spectrum reuse through the deployment of more access points per square mile has the potential to successfully meet the increasing demand for more bandwidth. In theory, the best approach to density increase is via distributed multiuser MIMO, where several access points are connected to a central server and operate as a large distributed multi-antenna access point, ensuring that all transmitted signal power serves the purpose of data transmission, rather than creating "interference." In practice, while enterprise networks offer a natural setup in which distributed MIMO might be possible, there are serious implementation difficulties, the primary one being the need to eliminate phase and timing offsets between the jointly coordinated access points. In this paper we propose AirSync, a novel scheme which provides not only time but also phase synchronization, thus enabling distributed MIMO with full spatial multiplexing gains. AirSync locks the phase of all access points using a common reference broadcasted over the air in conjunction with a Kalman filter which closely tracks the phase drift. We have implemented AirSync as a digital circuit in the FPGA of the WARP radio platform. Our experimental testbed, comprised of two access points and two clients, shows that AirSync is able to achieve phase synchronization within a few degrees, and allows the system to nearly achieve the theoretical optimal multiplexing gain. We also discuss MAC and higher layer aspects of a practical deployment. To the best of our knowledge, AirSync offers the first ever realization of the full multiuser MIMO gain, namely the ability to increase the number of wireless clients linearly with the number of jointly coordinated access points, without reducing the per client rate.

==> synchronization.tex <==

\section{Synchronization}


As mentioned in the introduction, various high-precision
synchronization schemes have been developed for industrial use. Some
of them make use of the Ethernet wired network as a transmission
medium, managing to deliver a timing reference accurate to within
10ns. A radio cirqcuit having a carrier circuit of 1 GHz, however,
suffers a complete phase excursion for every nanosecond difference in
the timing reference. It results that, for accurate transmission that
makes use of phase coherence, the phase jitter must be well in the
subnanosecond range.

Maintining a phase lock on a signal generated using a different time
reference is an integral part of every digital communication system,
be it one that simply uses a phase modulation such as QPSK or QAM or
an OFDM system which uses pilots in order to realize the
phase-tracking. The two modulations mentioned are also ssociated with
the two most common ways of acquiring the information for a phase
lock: in the case of simple phase modulation, the system selects a
time interval for which the phase is kept constant (a symbol) and uses
its phase as a reference. The phase is compared to the nearest
transmit constellation point and the difference is used as an
indicator of the time lag between the clocks of the transmitter and
receiver component. The difference is compensated for and the time
interval corresponding to the next symbol is so shifted in order to
align (in the long run) the shape of the received constellation over
the shape of the transmit constellation. In the case of an OFDM
modulation there are multiple pilot carriers whose phase is known both
to the transmitter and the receiver, and their phase deviations are
jointly used in order to determing the timing offset for the received
frame.

Assuming that the set of access points used as a virtual MIMO
transmission system has a central host acting as a clock reference, we
could implement such a phase-lock circuit in all the other hosts. Our
system proposes using the measured timing derived from the phase lock
on the main transmitter as an indication of the phase adjustments
needed in order to be sending signals that are phase-aligned with the
ones of the main transmitter. Naturally, obtaining a phase reference
from a received signal while transmitting another signal can be quite
a daunting task. The solutions are either using interference
cancellation or ensuring thatthe transmission of data used in the
synchronization procedure takes place in a time or frequency domain
uncluttered by secondary transmissions. Achieving separation in the
time domain leads us to a time-division strategy, whose key
determining parameter is the on/off switch time of the secondary
transmitter. Depending on the achievable times, synchronization data
could be either inserted within every frame (as a supplement to the
cyclic prefix) or every few frames, as a separate frame entirely. In
the frequency domain the crucial parameter is the roloff of the data
transmission band, which determines the bandwidth separation needed
between the data band and the time synchronization band.

This section would not be complete without an estimation of the
synchronization precission achievable. While exact time reference
transmission over the Ethernet is impossible, two reference clocks
paced by an Ethernet time synchronization protocol can be brought,
according to numerous sources, to a relative drift smaller than 1ppm
(part per million). Assuming that every OFDM frame has 4us length, as
is the case for example in 802.11, and that each frame is used as a
reference for the transmission of the next frame at the secondary, the
clock drift between the two sources can be bound to 0.004ns. Given a
carrier frequency of 2.4 GHz, this translates to a phase jitter of
less than 1\%. Using a simple precoding strategy such as zero-forcing,
it can be shown that the attenuation of interference, even for a
jitter of 10 degrees, or 2.7\% will be of about 20 dB, making it
comparable to the receiver noise.


==> then.tex <==
\label{section:then}
In THP the mapping
from the data symbol vector $\uv$ to the transmitted symbol vector $\xv$ is {\em non-linear}.
Consider again the channel model (\ref{eqn:channelmodel}).
THP imposes a given precoding ordering, 
and it pre-cancels sequentially the interference of already precoded signals. 
Without loss of generality, consider
the natural precoding ordering to be from $1$ to $K$, and let $\hv_k$ denote the 
$k$-th client's $M \times 1$ channel vector. 
Let $\Hm = \Qm \Rm$ be the QR factorization of $\Hm$, 
such that $\Rm$ is $K \times K$ upper triangular with real
non-negative diagonal coefficients, and $\Qm$ is such that $\Qm^\herm \Qm = \Id$. 
THP precoding is formed by the concatenation of a linear mapping, defined by the unitary matrix $\Qm$, 
with a non-linear mapping that does the interference pre-cancellation. 
Let $\hat{\uv} = {\rm THP}(\uv)$ denote the 
non-linear mapping of the data vector $\uv$ into an intermediate vector $\hat{\uv}$, that will be defined later. 
The linear mapping component of THP is then given by 
\begin{equation} 
\xv = \Qm \Sigmam^{1/2} \hat{\uv}, 
\end{equation}
where $\Sigmam = \diag(q_1,\ldots, q_K)$, and $q_k$ is the power allocated to the $k$-th stream. 
It follows that the channel reduces to
%\begin{eqnarray} \label{marameo1}
$\yv 
%& = & 
%\Hm^\herm \xv + \zv \nonumber \\
%& = & \Rm^\herm \Qm^\herm \Qm \Sigmam^{1/2} \hat{\uv} + \zv \nonumber\\
= \Lm \Sigmam^{1/2} \hat{\uv} + \zv$, 
%\end{eqnarray}
where $\Lm = \Rm^\herm$ is lower triangular. 
The signal seen at client $k$ receiver is given by 
\begin{equation} \label{channel-without-precoding} 
y_k = [\Lm]_{k,k} \sqrt{q_k} \hat{u}_k + \underbrace{\sum_{j < k} [\Lm]_{k,j} \sqrt{q_j} \hat{u}_j}_{\mbox{interference}} + z_k 
\end{equation}
Next, we look at the non-linear mapping $\uv \mapsto \hat{\uv}$. The goal is to pre-cancel the term 
indicated by ``interference'' in Equation \ref{channel-without-precoding}. Notice that this term depends only
on symbols $\hat{u}_j$ with $j < k$. Therefore, the elements $\hat{u}_1, \ldots, \hat{u}_K$ can be calculated sequentially. 
A simple pre-subtraction of the interference term at each step would increase the effective transmit power.

The key idea of THP is to introduce a modulo operation that limits the transmit power of each precoded stream
$\hat{u}_k$. This is defined as follows. Assume that the data symbols $u_k$ are points from a QAM constellation 
uniformly spaced in the squared region of the complex plane bounded by the interval $[-\tau/2, \tau/2]$ on both the real axis 
and the imaginary axis. 
Then, for a complex number $s$, let $s$ modulo $\tau$ be given by 
$[s]_{{\rm mod} \; \tau} = s - Q_\tau(s)$, where $Q_\tau(s)$ is the point $(n + jm)\tau$ with integers $n,m$ closest to $s$. 
In short, $Q_\tau(s)$ is the quantization of $s$ with respect to a square grid with minimum distance $\tau$ on the complex plane, 
and $[s]_{{\rm mod} \; \tau}$ is the quantization error. We let
\begin{equation} \label{minchiata}
\hat{u}_k = \left [ u_k - \frac{\sum_{j < k} [\Lm]_{k,j} \sqrt{q_j} \hat{u}_j}{[\Lm]_{k,k} \sqrt{q_k}} \right ]_{{\rm mod} \; \tau}.
\end{equation}
In this way, the symbol $\hat{u}_k$ is necessarily bounded into the squared region of side $\tau$, 
and its variance (assuming a uniform distribution over the squared region, which is approximately true when we use a QAM constellation inscribed in the square)
is given by $\EE[|\hat{u_k}|^2] = \tau^2/6$. Letting $\tau = \sqrt{6}$ we have that the precoded symbols have unit energy
and that the transmit power for stream $k$ is exactly given by $q_k$. 

Let's focus now on receiver $k$ and see how the modulo precoding can be undone. 
The receiver scales the received symbol $y_k$ by $[\Lm]_{k,k} \sqrt{q_k}$ and applies again the same the modulo $\tau$ non-linear mapping. 
Simple algebra then shows that 
\begin{eqnarray} \label{thp-receiver}
\widehat{y}_k & = & \left [ u_k + \frac{z_k}{[\Lm]_{k,k} \sqrt{q_k} } \right ]_{{\rm mod} \; \tau}.
\end{eqnarray}
It follows that the interference term is perfectly removed, but we have introduced a distortion in the noise term. 
Namely, while $u_k$ is unchanged by the modulo operation, since by construction it is a point inside the square, 
the noise term $\frac{z_k}{[\Lm]_{k,k} \sqrt{q_k} }$ is ``folded'' by the modulo operation, i.e., the tails of the Gaussian noise distribution
are folded on the squared region. Noise folding is a well-known effect of THP \cite{forney-eyuboglu}. 

As far as the achievable rate is concerned, it is possible to show (see \cite{tosato-boccardi-caire,erez-zamir-shamai}) that this is given by 
\begin{equation} \label{achievable-lowerbound-thp-i}
R_{\rm sum}^{\rm thp}(\SNR) = \sum_{k=1}^K \left [ \log(1 + |[\Lm]_{k,k}|^2 q_k) - \log (\pi e/6) \right ]_+,
\end{equation}
where $[\cdot]_+$ indicates the positive part. Again, this sum rate can be optimized with respect to the power allocation
$q_1, \ldots, q_K$, subject to the sum power constraint $\sum_{k=1}^K q_k \leq \SNR$. 
The rate penalty term $\log (\pi e/6)$ is the shaping loss, due to the fact that THP produces a signal which is uniformly 
distributed in the square region
(therefore, a codeword of $n$ signal components is uniformly distributed in an $n$-dimensional complex hypercube).
\footnote{It should be noticed that the same shaping loss is incurred by any other scheme such as
ZFBF, BIA, as well as TDMA if practical QAM constellations are used instead of the theoretical Gaussian coding ensemble.}



